Two Results on Slime Mold Computations

We present two results on slime mold computations. In wet-lab experiments (Nature'00) by Nakagaki et al. the slime mold Physarum polycephalum demonstrated its ability to solve shortest path problems. Biologists proposed a mathematical model, a system of differential equations, for the slime's adaption process (J. Theoretical Biology'07). It was shown that the process convergences to the shortest path (J. Theoretical Biology'12) for all graphs. We show that the dynamics actually converges for a much wider class of problems, namely undirected linear programs with a non-negative cost vector. Combinatorial optimization researchers took the dynamics describing slime behavior as an inspiration for an optimization method and showed that its discretization can $\varepsilon$-approximately solve linear programs with positive cost vector (ITCS'16). Their analysis requires a feasible starting point, a step size depending linearly on $\varepsilon$, and a number of steps with quartic dependence on $\mathrm{opt}/(\varepsilon\Phi)$, where $\Phi$ is the difference between the smallest cost of a non-optimal basic feasible solution and the optimal cost ($\mathrm{opt}$). We give a refined analysis showing that the dynamics initialized with any strongly dominating point converges to the set of optimal solutions. Moreover, we strengthen the convergence rate bounds and prove that the step size is independent of $\varepsilon$, and the number of steps depends logarithmically on $1/\varepsilon$ and quadratically on $\mathrm{opt}/\Phi$.

==> preliminaries.tex <==
% !TEX root = main.tex

\section{Preliminaries}\label{preliminaries}
Note that we may assume that $A$ has full row-rank since any equation that is linearly dependent on other equations can be deleted without changing the feasible set. We continue to use $n$ and $m$ for the dimension of $A$. Thus $A$ has rank $n$. We continue by fixing some terms and notation.
A \emph{basic feasible solution} of $Af = b$ is a vector $f = (f_B, f_N)$, where $f_B = A_B^{-1} b$ and $A_B$ is a square $n \times n$ non-singular sub-matrix of $A$ and and $f_N = 0$ is the vector indexed by the coordinates not in $B$. A feasible solution $f$ is \emph{kernel-free} or \emph{non-circulatory}  if it is contained in the convex hull of the basic feasible solutions.\footnote{For the undirected shortest path problem, we drop the equation corresponding to the sink. Then $b$ becomes the negative indicator vector corresponding to the source node. Note that $n$ is one less than the number of nodes of the graph.
The basic feasible solutions are the simple undirected source-sink paths. A circulatory solution contains a cycle on which there is flow.}
For a given capacity vector $x$ and a vector $f \in \R^m$ with $\supp(f) \subseteq \supp(x)$, we use $E(f) = \sum_e (c_e/x_e) f_e^2$ to denote the \emph{energy} of $f$. The energy of $f$ is infinite, if $\supp(f) \not\subseteq \supp(x)$. We use $\cost(f)= \sum_e c_e \abs{f_e} = c^T \abs{f}$ to denote the \emph{cost} of $f$.
 Note that $E(x) = \sum_e c_e x_e = \cost(x)$. 
We say that a vector $f'$ is \emph{sign-compatible} with a vector $f$ (of the same dimension) or $f$-sign-compatible if $f'_e \not= 0$ implies $f'_e f_e > 0$. In particular, $\supp(f') \subseteq \supp(f)$.
We use the constants
$\cmax = \|c\|_\infty$ and $\cmin = \min_{e:c_e > 0} c_e$. 
% We denote by $\D$ be the largest absolute value of a determinant of a square sub-matrix of $A$.

\subsection{A Corollary of the Finite Basis Theorem}
% A \emph{polyhedron} in $\mathbb{R}^{m}$ is the intersection
% of finitely many halfspaces, i.e.,the set $\{x\ |\ Ax\leq b\}$ is a polyhderon. A \emph{polydedral
% cone} in $\mathbb{R}^{m}$ is generated by a finite set of vectors
% $X$ such that $\{x=\sum_{i}\lambda_{i}x_{i}\ |\ x_{i}\in X,\ \lambda_{i}\geq0\}=\{x\ |\ Ax\leq0\}$,
% i.e. it is the intersection of finitely many halfspaces that contain
% the origin. A bounded polyhedron is called a polytope.
% 
% \begin{fact}\label{fact_Schrijver} \cite{Schrijver:book86}
%     A polyhedron $P=\{x\ |\ Ax\leq b\}$
%     can be written as the Minkowski sum of a polytope $Q$ and a cone
%     $C$ such that $P=Q+C=\{x+y\ |\ x\in Q,\ y\in C\}$.
% \end{fact}

% \begin{corollary}(Canonical Representation) \label{cor_Schrijver}
%     Every feasible vector
%     $f$, i.e. $Af=b$ and $f\geq0$, admits a representation $f=\sum_{i=1}^{m_{1}}\alpha_{i}f^{(i)}+\sum_{j=1}^{m_{2}}\beta_{j}\gamma^{(j)}$,
%     where $\alpha_{i},\beta_{j}\geq0$, $\sum_{i=1}^{m_{1}}\alpha_{i}=1$
%     and $\sum_{j=1}^{m_{2}}\beta_{j}\geq0$. Equivalently, $f$ can be
%     expressed as a summation over a convex combination of basic feasible
%     solutions ($Af^{(i)}=b$ and $f^{(i)}\geq0$) and a conical combination
%     of non-negative spanning vectors ($A\gamma^{(j)}=0$ and $\gamma^{(j)}\geq0$)
%     of the polyhedral cone of $A$.
% \end{corollary}
% A feasible vector $y$ is called \emph{kernel-free}, if it can be
% represented with vectors $\alpha\neq0$ and $\beta=0$, i.e. it is
% a convex combination of basic feasible solutions.

We use the following corollary of the finite basis theorem for polyhedra.

\begin{lemma}\label{sign-compatible representation}
	Let $f$ be a feasible solution to $Af=b$. Then $f$ is the sum of a convex combination of at most $n$ basic feasible solutions plus a vector in the kernel of $A$. Moreover, all elements in this representation are sign-compatible with $f$.
\end{lemma}
\begin{proof} We may assume $f \ge 0$. Otherwise, we flip the sign of the appropriate columns of $A$. Thus the system $Af =b,\ f \ge 0$ is feasible and $f$ is the sum of a convex combination of at most $n$ basic feasible solutions plus a vector in the kernel of $A$ by the finite basis theorem~\cite[Corollary 7.1b]{Schrijver:book86}. By definition, the elements in this representation are non-negative vectors and hence sign-compatible with $f$.
\end{proof}

Note that the above lemma also yields that a feasible solution to the directed linear program, i.e., a solution $f$ with $Af=b$ and $f\ge 0$ admits a decomposition into \emph{non-negative} basic feasible solutions and a \emph{non-negative} vector in the kernel of $A$. \KM{isn't this just rephrasing}.

\subsection{The Minimum Energy Solution}\label{subsec:MinEnergySol}

In this section, we derive properties of the minimum energy solution. In particular, if every nonzero vector in the kernel of $A$ has positive cost, 
\begin{compactenum}[\mbox{}\hspace{\parindent}(i)]
\item the minimum energy feasible solution is kernel-free and unique (Lemma~\ref{q is kernel-free}),
\item $\abs{q_e} \le \onenorm{b} \D$ for every $e$ (Lemma~\ref{upper bound on q}), 
\item $q$ is defined by~\lref{explicite pq} (Lemma~\ref{formula for $q$, general case}), and
\item $E(q) = b^T p$, where $p$ is defined by~\lref{explicite pq} (Lemma~\ref{$E(q) = b^T p$, general case}).
\end{compactenum}
For positive cost vector $c > 0$, these results are known. 

\begin{lemma}\label{q is kernel-free}
	If every nonzero vector in the kernel of $A$ has positive cost, the minimum energy feasible solution is kernel-free and unique.
\end{lemma}
\begin{proof} Let $q$ be a minimum energy feasible solution. Since $q$ is feasible, it can be written as $q_n + q_r$, where $q_n$ is a convex combination of basic feasible solutions and $q_r$ lies in the kernel of $A$. Moreover, all elements in this representation are sign-compatible with $q$ by Lemma~\ref{sign-compatible representation}. If $q_r \not= 0$, the vector
	$q - q_r$ is feasible and has smaller energy, a contradiction. Thus $q_r = 0$.

	We next prove uniqueness. Assume for the sake of a contradiction that there are two distinct minimum energy feasible solutions $\qone$ and $\qtwo$. We show that the solution $(\qone + \qtwo)/2$ uses less energy than $\qone$ and $\qtwo$. Since $h \mapsto h^2$ is a strictly convex function from $\R$ to $\R$, the average of the two solutions will be better than either solution if there is an edge $e$ with $r_e > 0$ and $\qone_e \not= \qtwo_e$. The difference
	$z = \qone - \qtwo$ lies in the kernel of $A$ and hence $\cost(z) = \sum_e c_e \abs{z_e} > 0$. Thus there is an $e$ with $c_e > 0$ and $z_e \not= 0$. We have now shown uniqueness.
\end{proof}

\begin{lemma}\label{upper bound on q} Assume that every nonzero vector in the kernel of $A$ has positive cost. Let $q$ be the minimum energy feasible solution. Then $\abs{q_e}  \le \onenorm{b} \D$ for every $e$.
\end{lemma}
\begin{proof} Since $q$ is a convex combination of basic feasible solutions, $\abs{q_e} \le \max_z \abs{z_e}$
	where $z$ ranges over basic feasible solutions. Any basic feasible solution is of the form $(z_B,0)$, where $z_B = A_B^{-1} b$ and $A_B$ is a $n\times n$ non-singular submatrix of $A$. Thus every component of $z$ is bounded by $\onenorm{b} \D$.
\end{proof}

In~\cite{SV-LP}, the bound $|q_e|\le \D^2 m \onenorm{b}$ was shown.
We will now derive explicit formulae for the minimum energy solution $q$. We will express $q$ in terms of a vector $p \in \R^n$, which we refer to as the \emph{potential}, by analogy with the network setting, in which $p$  can be interpreted as the electric potential of the nodes. 
The energy of the minimum energy solution is equal to $b^T p$.
We also derive a local Lipschitz condition for the mapping from $x$ to $q$. Note that for $c> 0$ most of these facts are well-known.
% We treat positive cost vectors in Section~\ref{positive cost vector} and general cost vectors in Section~\ref{general cost vector}.


% In the undirected shortest path problem, $r_e q_e$ is the potential difference across the edge $e$. Since $r_e q_e = A_e^T L^{-1} b = A_e^T p$ we refer to $A_e^T p$ as the \emph{potential difference} across $e$. We also refer to $p$ as the \emph{potential}.

% \subsubsection{Positive Cost Vector}\label{positive cost vector}
% For completeness, we include a proof for the following facts in the appendix.
% \begin{fact}\label{formula for q}
% 	Assume $c > 0$ and let $r_e = c_e/x_e$, $R = \diag(r)$, and $p = (A R^{-1} A^T)^{-1} b$.
% 	\begin{compactenum}
% 		\item  Then $q = R^{-1} A^T p$ is the unique minimum energy feasible solution.
% 		\item Let $f$ be any feasible solution. Then $E(q) = b^T p = f^T A^T p$.
% 	\end{compactenum}
% \end{fact}
%
% % \begin{proof} Since $x > 0$ and $c > 0$, the diagonal elements of $R$ are positive. Thus $R = S \cdot S = S^T S$ for the diagonal matrix $S = R^{1/2}$ having the values $\sqrt{r_e}$ on the diagonal. Thus $A R^{-1} A^T = A S^{-1} (A S^{-1})^T$ and hence for a vector $r$, $r^T A R^{-1} A^T r = 0$ only if $r^T A S^{-1} = 0$ only if $r^T A = 0$ only if $r^T = 0$. The last equivalence requires that $A$ has full rank. Thus $p$ and hence $q$ exists.
% %
% % The KKT conditions state that the minimizer of the energy must satisfy $R q = A^T p$ for some $p$. Note that $2Rf$ is the gradient of the energy with respect to $f$ and that the $e$-th column of $A$ is the gradient of the $A f = b$ with respect to $f_e$. We may absorb the factor $2$ in the $p$. Thus $q = R^{-1} A^T p$. Since $q$ is a feasible flow, we must also have $b = Aq = A R^{-1} A^T p$.
% % \end{proof}
%
% % \begin{lemma}\label{$E(q) = b^T p$} Assume $c > 0$. Let $q$ be the minimum energy feasible solution and let $f$ be any feasible solution. Then $E(q) = b^T p = f^T A^T p$. \end{lemma}
% % \begin{proof}
% % By definition,
% % \[ E(q) = q^T R q = p^T A R^{-1} R q = p^T A q = p^T b.\]
% % Also, $f^T A^T p = (Af)^T p = b^T p$. \end{proof}
%
% How does reorienting a column of $A$ affect $p$ and $q$? Say we reorient the $e$-th column of $A$. This flips the sign of $q_e$. Since $q_e = (x_e/c_e) A_e^T p$, the sign flips of $q_e$ and $A_e^T$ cancel and the same $p$ works. Thus reorienting the columns of $A$ has NO effect on $p$.
% We will next study more closely, how $p$ and $q$ depend on $x$. In particular, we will show that the mapping $x \mapsto q$ is locally Lipschitz. The proof  uses Cramer's rule and the Cauchy-Binet formula. Note that for the undirected shortest path problem the Cauchy-Binet formula specializes to Kirchhoff's spanning tree theorem, see~\cite[Section 5]{Physarum}. We include the proof in the main part of the paper, because we consider the application of the Cauchy-Binet formula interesting.
% \begin{lemma}\label{Locally Lipschitz}
% 	Assume $c > 0$ and that $A$, $b$, and $c$ are integral. Let $\delta > 0$ and $d > 0$.
% 	Then for any $e \in [m]$ and any two vectors $x$ and $\tilde{x}$ in $\R^m$ with $\delta \bfone \le x, \tilde{x} \le d \bfone$, define $M = 2 m^n (d/\delta)^n \cmax^n \D^2 \onenorm{b}$. Then, it holds that
% 	$\abs{\abs{q_e(x)} - \abs{q_e(\tilde{x})}} \le M \infnorm{x - \tilde{x}}$.
% 	% where $M = 2 m^n (d/\delta)^n \cmax^n \D^2 \onenorm{b}$.
% 	%\[    \abs{ \frac{\partial q_e}{\partial x_i}}\le  2 m^n (d/\delta)^n \cmax^n \D^2 \onenorm{b}. \]
% \end{lemma}
% \begin{proof} Recall that Cramer's rule yields
% 	\[              (A R^{-1} A^T)^{-1} = \frac{1}{\det (A R^{-1} A^T)} ( (-1)^{i+j} \det M_{-j,-i})_{ij}, \]
% 	where $M_{-i,-j}$ is obtained from $A R^{-1} A^T$ by deleting the $i$-th row and the $j$-th column. For a subset $S$ of $[m]$ and an index $i \in [n]$, let $A_S$ be the $n \times \abs{S}$ matrix consisting of the columns selected by $S$ and let $A_{-i,S}$ be the matrix obtained from $A_S$ by deleting row $i$. If $D$ is a diagonal matrix of size $m$, then $(A D)_S = A_S D_S$. The Cauchy-Binet theorem expresses the determinant of a product of two matrices (not necessarily square) as a sum of determinants of square matrices. It yields
% 	\begin{align*}
% 		\det (A R^{-1} A^T)
% 		% &= \det(A R^{-1/2} (A R^{-1/2})^T )
% 		= \sum_{S \subseteq [m];\ \abs{S} = n} (\det( (AR^{-1/2})_S))^2
% 		% &= \sum_{S \subseteq [m];\ \abs{S} = n} (\det(A_S \cdot R^{-1/2}_S ))^2
% 		% = \sum_{S \subseteq [m];\ \abs{S} = n} (\det A_S)^2  \cdot (\det R^{-1/2}_S)^2                                                                                   \\
% 		= \sum_{S \subseteq [m];\ \abs{S} = n} (\prod_{e \in S} x_e/c_e) \cdot  (\det A_S)^2.
% 	\end{align*}
% 	Similarly,
% 	\begin{align*}
% 		\det (A R^{-1} A^T)_{-i,-j}
% 		% &= \det((A R^{-1/2})_{-i} (A R^{-1/2})_{-j}^T )
% 		% = \sum_{S \subseteq [m];\ \abs{S} = n-1} \det( (AR^{-1/2})_{-i,S}) \cdot   \det( (AR^{-1/2})_{-j,S}) \\
% 		% &= \sum_{S \subseteq [m];\ \abs{S} = n-1} \det(A_{-i,S} \cdot R^{-1/2}_S ) \cdot  \det(A_{-j,S} \cdot R^{-1/2}_S )\\
% 		  & = \sum_{S \subseteq [m];\ \abs{S} = n-1} (\prod_{e \in S} x_e/c_e) \cdot  (\det A_{-i,S} \cdot \det A_{-j,S}).
% 	\end{align*}
% 	Thus using $p = (A R^{-1} A^T)^{-1} b$, we obtain
% 	\begin{equation}\label{explicite p}
% 		p_i = \frac{\sum_{j \in [n]} (-1)^{i + j}\sum_{S \subseteq [m];\ \abs{S} = n-1} (\prod_{e \in S} x_e/c_e) \cdot  (\det A_{-i,S} \cdot \det A_{-j,S}) b_j }{\sum_{S \subseteq [m];\ \abs{S} = n} (\prod_{e \in S} x_e/c_e) \cdot  (\det A_S)^2},
% 	\end{equation}
% 	and using $q = R^{-1} A^T p$, this yields
% 	\begin{align}\label{explicite q}
% 		q_e
% 		= \frac{\sum_{S \subseteq [m];\ \abs{S} = n-1} (\prod_{e' \in S\cup e} x_{e'}/c_{e'}) \cdot  \det (A_S | A_e) \cdot \det (A_S | b) }{\sum_{S \subseteq [m];\ \abs{S} = n} (\prod_{e' \in S} x_{e'}/c_{e'}) \cdot  (\det A_S)^2},
% 	\end{align}
% 	where $(A_S| A_e)$, respectively $(A_S | b)$, denotes the $n \times n$ matrix whose columns are selected from $A$ by $S$ and whose last column is equal to $A_e$, respectively $b$. A more detailed derivation of~\eqref{explicite q} can be found in the appendix.
%
% 	We are now ready to estimate the derivative $\partial q_e/\partial x_i$. Assume first that $e \not= i$. By the above,
% 	$q_e = \frac{x_e}{c_e} \frac{F + G x_i/c_i}{H + I x_i/c_i}$,
% 	where $F$, $G$, $H$ and $I$ are given implicitly by \eqref{explicite q}. Then
% 	\[    \abs{\frac{\partial q_e}{\partial x_i}} =  \abs{\frac{x_e}{c_e} \frac{ FI/c_i -  GH/c_i} {(H + I x_i/c_i)^2}} \le \frac{ 2 \cdot {\binom{m}{n - 1}} d^n \D^2 \onenorm{b}}{ (\delta/\cmax)^{n}} \le M.\]
% 	For $e = i$, we have
% 	$q_e = \frac{G x_e/c_e}{H + I x_e/c_e}$,
% 	where $G$, $H$, and $I$ are given implicitly by \eqref{explicite q}. Then
% 	\[    \abs{\frac{\partial q_e}{\partial x_e}} =  \abs{\frac{GH/c_e} {(H + I x_e/c_e)^2}} \le \frac{{\binom{m}{n - 1}} d^{n} \D^2 \onenorm{b}}{ (\delta/\cmax)^{n}} \le M.\]
% 	Finally, consider $x$ and $\tilde{x}$ with $\delta \bfone \le x, \tilde{x} \le d \bfone$. Let $\bar{x}_\ell = (\tilde{x}_1, \ldots, \tilde{x}_\ell, x_{\ell + 1}, \ldots, x_m)$. Then
% 	\[ \abs{\abs{q_e(x)} - \abs{q_e(\tilde{x})}} \le \abs{q_e(x) - q_e(\tilde{x})} \le \sum_{0 \le \ell < m} \abs{q_e(\bar{x}_\ell) - q_e(\bar{x}_{\ell + 1})} \le M \onenorm{x - \tilde{x}}. \qedhere\]
% \end{proof}



% \subsubsection{General Cost Vector}\label{general cost vector}
% We turn to the case of a general cost vector $c\ge 0$ with possibly vanishing entries.
% A proof of the following lemma can be found in the appendix.

\begin{lemma}\label{formula for $q$, general case}
	Assume that every nonzero vector in the kernel of $A$ has positive cost. Let $r_e = c_e/x_e$ and let $R$ denote the corresponding diagonal matrix. Let us split $[m]$ into $Z = \set{e}{c_e = 0}$ and $P = E \setminus Z$, similarly $A$ into $A_P$ and $A_Z$ and $q$ into $q_P$ and $q_Z$.  Since $A_Z$ has linearly independent columns, we may assume that the first $\abs{Z}$ rows of $A_Z$ form a square non-singular matrix. We can thus write $A=\big[\begin{smallmatrix}A'_P & A'_Z \\ A''_P & A''_Z \end{smallmatrix}\big]$ with invertible $A'_Z$. Then the minimum energy solution satisfies 
	\begin{equation}\label{both blocks}
		\begin{bmatrix} A'_P & A'_Z  \\ A''_P & A''_Z \end{bmatrix}
		\begin{bmatrix} q_P \\ q_{Z} \end{bmatrix}
		= \begin{bmatrix} b' \\ b'' \end{bmatrix} 
% Then the minimum energy feasible solution satisfies
% 	\begin{align}\label{both blocks}
% 		\begin{bmatrix} A_P & A_Z \end{bmatrix}
% 		\begin{bmatrix} q_P \\ q_{Z} \end{bmatrix}
% 		= b
		\quad\text{ and }\quad
		\begin{bmatrix} R_P &   \\  & 0 \end{bmatrix}
		\begin{bmatrix} q_{P} \\ q_{Z} \end{bmatrix}  =
		\begin{bmatrix} {A'_P}^T & {A''_P}^T\\ {A'_Z}^T & {A''_Z}^T \end{bmatrix}  \begin{bmatrix} p' \\ p'' \end{bmatrix}
\end{equation}
%	\end{align}
for some vector $p = \big[ \begin{smallmatrix} p' \\ p'' \end{smallmatrix} \big]$; here $p'$ has dimension $\abs{Z}$. The equation system~\eqref{both blocks} has a unique solution given by 
	\begin{align}\label{explicite pq}
		\begin{bmatrix} q_Z                         \\q_P\end{bmatrix}
		=\begin{bmatrix}[A'_Z]^{-1} (b' - A'_P q_P) \\ R_P^{-1} A^T_P p\end{bmatrix}
		\quad \text{ and }\quad
		\begin{bmatrix} p'                          \\p''\end{bmatrix}
		=\begin{bmatrix}- [A'_Z]^{-T} [A''_Z]^T p'' \\MR^{-1}M^T (b'' - A''_Z [A'_Z]^{-1} b')\end{bmatrix},
	\end{align}
	where $M= A''_P  - A''_Z (A'_Z)^{-1} A'_P$ is the Schur complement of the block $A'_Z$ of the matrix $A$.
\end{lemma}

\begin{proof}  $q$ minimizes $E(f) = f^T R f$ among all solutions of $Af = b$. The KKT conditions state that $q$ must satisfy $R q = A^T p$ for some $p$. Note that $2Rf$ is the gradient of the energy $E(f)$ with respect to $f$ and that the $-A^Tp$ is the gradient of $p^T(b - A f)$ with respect to $f$. We may absorb the factor $-2$ in $p$. Thus $q$ satisfies \eqref{both blocks}. 

We show next that the linear system \eqref{both blocks} has a unique solution. The top $\abs{Z}$ rows of the left system in~\eqref{both blocks} give
	\begin{equation}\label{expression for qZ}
		q_Z = [A'_Z]^{-1} (b' - A'_P q_P).
	\end{equation}
	Substituting this expression for $q_Z$ in into the bottom $n - \abs{Z}$ rows of the left system in~\eqref{both blocks} yields
	\[ M  q_P = b'' - A''_Z (A'_Z)^{-1} b'. \]
From the top $\abs{P}$ rows of the right system in~\eqref{both blocks} it holds that
	$q_P = R_P^{-1} A^T_P \cdot p$.
Thus
	\begin{equation}\label{equation for p}
		M R_P^{-1} A^T_P \cdot p = b'' - A''_Z [A'_Z]^{-1} \cdot b'.
	\end{equation}
The bottom $n - \abs{Z}$ rows of the right system in~\eqref{second block} yield $0 = A_Z^T p = (A'_Z)^T p' + (A''_Z)^T p''$ and hence
	\begin{equation}\label{expression for pprime}
		p' = - [A'_Z]^{-T} [A''_Z]^T p''.
	\end{equation}
	Substituting~(\ref{expression for pprime}) into~\eqref{equation for p} yields
	\begin{align}
		b'' - A''_Z (A'_Z)^{-1} b' & =  MR_{P}^{-1}\left([A'_{P}]^{T}p'+[A''_{P}]^{T}p''\right) \notag
		\\ \nonumber
		                           & = MR_{P}^{-1}\left([A''_{P}]^{T}-[A'_{P}]^{T}(A'_{Z})^{-T}(A''_{Z})^{T}\right) p'' \\
		                           & = MR_P^{-1}M^T p''. \label{expression for pprimeprime}
	\end{align}
	It remains to show that the matrix $MR_P^{-1}M^T$ is non-singular. We first observe that the rows of $M$ are linearly independent. Consider the left system in \eqref{both blocks}. Multiplying the first $\abs{Z}$ rows by $(A'_Z)^{-1}$ and then subtracting $A''_Z$ times the resulting rows from the last $n - \abs{Z}$ rows turns $A$ into the matrix
	$
	Q=\big[\begin{smallmatrix}
		[A'_Z]^{-1} A'_P & I  \\ M & 0
	\end{smallmatrix}\big].
	$
	By assumption, $A$ has independent rows. Moreover, the preceding operations guarantee that $\rank(A)=\rank(Q)$. Therefore, $M$ has independent rows. Since $R_P^{-1}$ is a positive diagonal matrix, $R_P^{-1/2}$ exists and is a positive diagonal matrix. Let $z$ be an arbitrary nonzero vector of dimension $\abs{P}$. Then $z^T MR_P^{-1}M^Tz = (R_P^{-1/2} M^T z)^T (R_P^{-1/2} M^T z) > 0$ and hence  $MR_P^{-1}M^T$ is non-singular. It is even positive semi-definite. 


	There is a shorter proof that the system~\eqref{both blocks} has a unique solution. However, the argument does not give an explicit expression for the solution. In  the case of a convex objective function and affine constraints, the KKT conditions are sufficient for being a global minimum. Thus any solution to~\eqref{both blocks} is a global optimum. We have already shown in Lemma~\ref{q is kernel-free} that the global minimum is unique.
\end{proof}


We next observe that the energy of $q$ can be expressed in terms of the potential. 
%The following proof only uses that $q$ satisfies~\eqref{first block} and~\eqref{second block}. It does not use that the system defined by these equations has a unique solution.

\begin{lemma}\label{$E(q) = b^T p$, general case} Let $q$ be the minimum energy feasible solution and let $f$ be any feasible solution. Then $E(q) = b^T p = f^T A^T p$. \end{lemma}
\begin{proof}
	As in the proof of Lemma~\ref{formula for $q$, general case}, we split $q$ into $q_P$ and $q_Z$, $R$ into $R_P$ and $R_Z$, and $A$ into $A_P$ and $A_Z$. Then
	\begin{align*}
		E(q) & = q_P^T R_P q_P     & \text{by the definition of $E(q)$ and since $R_Z = 0$}                \\
		     & = p^T A_P q_p       & \text{by  the right system in~\eqref{both blocks}}  \\
		     & = p^T (b - A_Z q_Z) & \text{by the left system in~\eqref{both blocks}}                                  \\
		%    &= b^T p - p^T A_Z q_Z \\
		     & = b^T p             & \text{by the right system in~\eqref{both blocks}}.
	\end{align*}
	For any feasible solution $f$, we have $f^T A^T p = b^T p$.
\end{proof}

\subsection{Existence of a Solution to the Undirected Physarum Dynamics}

In this section we show that a solution $x(t)$ to~\eqref{PD} has domain $[0,\infty)$. We first show that the mapping $x \mapsto q$ is Lipschitz continuous; this implies existance by standard arguments. 
Our analysis builds upon Cramer's rule and the Cauchy-Binet formula. The Cauchy-Binet formula extends Kirchhoff's spanning tree theorem which was used in ~\cite{Physarum} for the analysis of the undirected shortest path problem. 

\begin{lemma}\label{Locally Lipschitz, General Case}
	Assume $c \ge 0$, no non-zero vector in the kernel of $A$ has cost zero, and that $A$, $b$, and $c$ are integral. Let $\alpha,\beta > 0$. For any $e \in [m]$ and any two vectors $x$ and $\tilde{x}$ in $\R^m$ with $\alpha \bfone \le x, \tilde{x} \le \beta \bfone$, define $\gamma = 2 m^n (\beta/\alpha)^n \cmax^n \D^2 \onenorm{b}$. Then $\big|\abs{q_e(x)} - \abs{q_e(\tilde{x})}\big| \le \gamma \infnorm{x - \tilde{x}}$.
\end{lemma}
\begin{proof}
	First assume that $c>0$. By Cramer's rule
	\[
		(A R^{-1} A^T)^{-1} = \frac{1}{\det (A R^{-1} A^T)} ( (-1)^{i+j} \det M_{-j,-i})_{ij},
	\]
	where $M_{-i,-j}$ is obtained from $A R^{-1} A^T$ by deleting the $i$-th row and the $j$-th column. For a subset $S$ of $[m]$ and an index $i \in [n]$, let $A_S$ be the $n \times \abs{S}$ matrix consisting of the columns selected by $S$ and let $A_{-i,S}$ be the matrix obtained from $A_S$ by deleting row $i$. If $D$ is a diagonal matrix of size $m$, then $(A D)_S = A_S D_S$. The Cauchy-Binet theorem expresses the determinant of a product of two matrices (not necessarily square) as a sum of determinants of square matrices. It yields
	\begin{align*}
		\det (A R^{-1} A^T)
		% &= \det(A R^{-1/2} (A R^{-1/2})^T )
		= \sum_{S \subseteq [m];\ \abs{S} = n} (\det( (AR^{-1/2})_S))^2
		% &= \sum_{S \subseteq [m];\ \abs{S} = n} (\det(A_S \cdot R^{-1/2}_S ))^2
		% = \sum_{S \subseteq [m];\ \abs{S} = n} (\det A_S)^2  \cdot (\det R^{-1/2}_S)^2                                                                                                                                                                      \\
		= \sum_{S \subseteq [m];\ \abs{S} = n} (\prod_{e \in S} x_e/c_e) \cdot  (\det A_S)^2.
	\end{align*}
	Similarly,
	\begin{align*}
		\det (A R^{-1} A^T)_{-i,-j}
		% &= \det((A R^{-1/2})_{-i} (A R^{-1/2})_{-j}^T )
		% = \sum_{S \subseteq [m];\ \abs{S} = n-1} \det( (AR^{-1/2})_{-i,S}) \cdot   \det( (AR^{-1/2})_{-j,S}) \\
		% &= \sum_{S \subseteq [m];\ \abs{S} = n-1} \det(A_{-i,S} \cdot R^{-1/2}_S ) \cdot  \det(A_{-j,S} \cdot R^{-1/2}_S )\\
		  & = \sum_{S \subseteq [m];\ \abs{S} = n-1} (\prod_{e \in S} x_e/c_e) \cdot  (\det A_{-i,S} \cdot \det A_{-j,S}).
	\end{align*}
Using $p = (A R^{-1} A^T)^{-1} b$, we obtain
	\begin{equation}\label{explicite p}
		p_i = \frac{\sum_{j \in [n]} (-1)^{i + j}\sum_{S \subseteq [m];\ \abs{S} = n-1} (\prod_{e \in S} x_e/c_e) \cdot  (\det A_{-i,S} \cdot \det A_{-j,S}) b_j }{\sum_{S \subseteq [m];\ \abs{S} = n} (\prod_{e \in S} x_e/c_e) \cdot  (\det A_S)^2}.
	\end{equation}
Substituting into $q = R^{-1} A^T p$ yields
	\begin{align}\label{explicite q}
		q_e
		  & = \frac{x_e}{c_e} A_e^T p                                                                                                                                                                                                                                                                                               \notag \\
		  & = \frac{x_e}{c_e} \sum_i A_{i,e} \cdot \frac{\sum_{j \in [n]} (-1)^{i + j +2n}\sum_{S \subseteq [m];\ \abs{S} = n-1} (\prod_{e' \in S} x_{e'}/c_{e'}) \cdot  (\det A_{-i,S} \cdot \det A_{-j,S}) b_j }{\sum_{S \subseteq [m];\ \abs{S} = n} (\prod_{e' \in S} x_{e'}/c_{e'}) \cdot  (\det A_S)^2} \notag                \\
		  & = \frac{\sum_{S \subseteq [m];\ \abs{S} = n-1}  \left((\prod_{e' \in S \cup e} x_{e'}/c_{e'}) \cdot \sum_{i \in [n]} (-1)^{i + n}A_{i,e} \det A_{-i,S} \cdot \sum_{j \in [n]}  (-1)^{j + n} b_j \det A_{-j,S}\right)}{\sum_{S \subseteq [m];\ \abs{S} = n} (\prod_{e' \in S} x_{e'}/c_{e'}) \cdot  (\det A_S)^2} \notag \\
		  & = \frac{\sum_{S \subseteq [m];\ \abs{S} = n-1} (\prod_{e' \in S\cup e} x_{e'}/c_{e'}) \cdot  \det (A_S | A_e) \cdot \det (A_S | b) }{\sum_{S \subseteq [m];\ \abs{S} = n} (\prod_{e' \in S} x_{e'}/c_{e'}) \cdot  (\det A_S)^2},
	\end{align}
	where $(A_S| A_e)$, respectively $(A_S | b)$, denotes the $n \times n$ matrix whose columns are selected from $A$ by $S$ and whose last column is equal to $A_e$, respectively $b$. 
%A more detailed derivation of~\eqref{explicite q} can be found in the appendix.

	We are now ready to estimate the derivative $\partial q_e/\partial x_i$. Assume first that $e \not= i$. By the above,
	$q_e = \frac{x_e}{c_e} \frac{F + G x_i/c_i}{H + I x_i/c_i}$,
	where $F$, $G$, $H$ and $I$ are given implicitly by \eqref{explicite q}. Then
	\[    \abs{\frac{\partial q_e}{\partial x_i}} =  \abs{\frac{x_e}{c_e} \frac{ FI/c_i -  GH/c_i} {(H + I x_i/c_i)^2}} \le \frac{ 2 \cdot {\binom{m}{n - 1}} \beta^n \D^2 \onenorm{b}}{ (\alpha/\cmax)^{n}} \le \gamma.\]
	For $e = i$, we have
	$q_e = \frac{G x_e/c_e}{H + I x_e/c_e}$,
	where $G$, $H$, and $I$ are given implicitly by \eqref{explicite q}. Then
	\[    \abs{\frac{\partial q_e}{\partial x_e}} =  \abs{\frac{GH/c_e} {(H + I x_e/c_e)^2}} \le \frac{{\binom{m}{n - 1}} \beta^{n} \D^2 \onenorm{b}}{ (\alpha/\cmax)^{n}} \le \gamma.\]
	Finally, consider $x$ and $\tilde{x}$ with $\alpha \bfone \le x, \tilde{x} \le \beta \bfone$. Let $\bar{x}_\ell = (\tilde{x}_1, \ldots, \tilde{x}_\ell, x_{\ell + 1}, \ldots, x_m)$. Then
	\[ \abs{\abs{q_e(x)} - \abs{q_e(\tilde{x})}} \le \abs{q_e(x) - q_e(\tilde{x})} \le \sum_{0 \le \ell < m} \abs{q_e(\bar{x}_\ell) - q_e(\bar{x}_{\ell + 1})} \le \gamma \onenorm{x - \tilde{x}}.
	\]
	In the general case where $c\ge 0$, we first derive an expression for $p''$ similar to~\eqref{explicite p}.
	Then the equations for $p'$ in~\eqref{explicite pq} yield $p'$, the equations for $q_P$ in~\eqref{explicite pq} yield $q_P$, and finally the equations for $q_Z$ in~\eqref{explicite pq} yield $q_Z$.
\end{proof}


We use Gr\"onwall's Lemma to derive bounds on a function from a differential inequality.
\begin{lemma}[Gr\"onwall's Lemma]\label{Gronwall}
	\begin{enumerate}
		\item Let $u(t)$ and $\beta(t)$ be functions satisfying $\dot{u}(t) \le \beta(t) u(t)$. Then $u(t) \le u(0) \cdot \exp(\int_0^t \beta(s)\ ds)$.
		In particular, choosing $\beta(t):=-1$ and $u(t):=-v(t)$ yields $v(t) \ge v(0) \cdot\exp(-t)$, if $\dot{v}(t) \ge - v(t)$.
		\item Let $Y(t)$ be a function satisfying $\dot{Y} \ge a - Y$ for some constant $a$. Then $Y(t) \ge a + (Y(0) - a)\exp(-t)$. Similarly, if
		      $\dot{Y} \le a - Y$, then $Y(t) \le a + (Y(0) - a)\exp(-t)$.
	\end{enumerate}
\end{lemma}
\begin{proof}
	The first part is a classical result, we only show the second part here. We have
	\[
		\frac{d}{ds}  Y(s) e^s = \dot{Y}(s) e^s + Y(s) e^s = (\dot{Y}(s) + Y(s))e^s \ge a \cdot  e^s,
	\]
	and hence by integrating on both sides from $0$ to $t$, we get
	$
	Y(t) e^t - Y(0) \ge a(e^t - 1)$. The bound on $Y(t)$ follows.
\end{proof}

\begin{lemma}\label{x is bounded}\label{existence}
	The solution to the undirected dynamics in~\eqref{PD} has domain $[0,\infty)$. Moreover,
	$x(0) e^{-t} \le x(t) \le  \onenorm{b} \D \bfone + \max(\bfzero, x(0) - \onenorm{b} \D \cdot \bfone) e^{-t}$ for all $t$.
\end{lemma}
\begin{proof}
	Consider any $x_0 > 0$ and any $t_0 \ge 0$. We first show that there is a positive $\delta'$ (depending on $x_0$) such that a unique solution $x(t)$ with $x(t_0) = x_0$ exists for $t \in (t_0 - \delta',t_0 + \delta')$. By the Picard-Lindel\"{o}f Theorem,	%\footnote{Let $x' = F(t,x)$ and $x(t_0) = x_0$.	If $F(t,x)$ is continuous on a region $R = \set{(t,x)}{t_0 - \delta < t < t_0 + \delta,\ \infnorm{x - x_0} < \epsilon}$ and satisfies a Lipschitz condition, i.e., for all $(t,x), (t,\tilde{x}) \in R$ $\abs{F(t,x) - F(t,\tilde{x}} \le L \cdot \norm{x - \tilde{x}}$ for some constant $L$, then there exists a $\delta' > 0$ such that the solution $x(t)$ with $x(t_0) = x_0$ exists and is unique for $t_0 - \delta' < t < t_0 + \delta'$.}
	this holds true if the mapping $x \mapsto \abs{q} - x$ is continuous and satisfies a Lipschitz condition in a neighborhood of $x_0$. Continuity clearly holds. Let $\epsilon = \min_i (x_0)_i/2$ and let $U = \set{x}{\infnorm{x - x_0} < \epsilon}$. Then for every $x, \tilde{x} \in U$ and every $e$
	\[
		\big|\abs{q_e(x)} - \abs{q_e(\tilde{x})}\big| \le \gamma \onenorm{x - \tilde{x}},
	\]
	where $\gamma$ is as in Lemma~\ref{Locally Lipschitz, General Case}.
	Local existence implies the existence of a solution which cannot be extended. Since $q$ is bounded (Lemma~\ref{upper bound on q}), $x$ is bounded at all finite times, and hence the solution exists for all $t$.
	The lower bound $x(t)  \ge x(0) e^{-t} > 0$ holds by Gr\"onwall's Lemma.
	Since $\abs{q_e} \le \onenorm{b} \D$, $\dot{x} = \abs{q} - x \le \onenorm{b} \D \bfone - x$. Thus, by the second part of Lemma~\ref{Gronwall}, we have $x(t) \le \onenorm{b} \D \bfone + \max(\bfzero, x(0) - \onenorm{b} \D \cdot \bfone) e^{-t}$.
\end{proof}

\subsection{LP Duality}\label{subsec:maxflowmincut}

The max-flow min-cut theorem plays an essential role in the analysis in~\cite{Physarum}. The proper generalization of max-flow to our situation is to consider the linear program $\max\{\alpha : Af = \alpha b, |f| \le x\}$, where $x$ is a fixed positive vector. Linear programming duality yields the corresponding minimization problem which generalizes the minimum cut problem to our situation. 

\begin{lemma}\label{dual}
    Let $x \in \R_{>0}^{m}$ and $b \not= 0$. The following linear programs 
	\begin{align}\label{LP-Duality}
		\max\{\alpha : Af = \alpha b, |f| \le x\}
		\qquad\qquad \min \{\abs{y^T A} x: b^Ty = -1\}
	\end{align}
are feasible and have the same objective value. 
	Moreover, there is a finite set $D = \sset{d^1,\ldots,d^K}$ of vectors $d^i \in \R_{\ge 0}^m$ that are independent of $x$ such that the minimum above is equal to $\Copt = \min_{d \in D} d^Tx$. There is a feasible $f$ with $\abs{f} \le x/\Copt$.\footnote{%
In the undirected shortest path problem, the $d$'s are the incidence vectors of the undirected source-sink cuts. Let $S$ be any set of vertices containing $s_0$ but not $s_1$, and let $\mathbf{1}^S$ be its associated indicator vector. The cut corresponding to $S$ contains the edges having exactly one endpoint in $S$. Its  indicator vector is  $d^S=\abs{A^T \mathbf{1}^S}$. Then $d^S_e = 1$ iff $\abs{S \cap \sset{u,v}} = 1$, where $e = (u,v)$ or $e = (v,u)$, and $d^S_e=0$ otherwise. For a vector $x \ge 0$, $(d^S)^T x$ is the capacity of the source-sink cut $(S,V\backslash S)$. 
In this setting, $\Copt$ is the value of a minimum cut. 
}
\end{lemma}
\begin{proof}
	\providecommand{\zn}{z^{-}}
	\providecommand{\zp}{z^{+}}
	$\alpha = 0$ and $f = 0$ is a feasible solution for the maximization problem. Since $b\neq 0$, there exists $y$ with $ b^Ty = -1$ and thus both problems are feasible. The dual of $\max\{\alpha:Af - \alpha b = 0,f \le x, -f \le x$
	has unconstrained variables $y \in \R^n$ and non-negative variables $\zp,\zn\in\R^m$ and reads
	\begin{equation} \label{dual LP}
		\min\{x^T (\zp + \zn) : - b^T y = 1, A^Ty + \zp - \zn = 0,\  \zp,\zn\ge 0\}.
	\end{equation}
	From $\zn = A^T y + \zp$, $\zp \ge 0$, $\zn \ge 0$ and $x > 0$, we conclude $\min(\zp,\zn) = 0$ in an optimal solution. Thus $\zn= \max(0, A^Ty)$  and $\zp= \max(0, -A^T y)$ and hence  $\zp + \zn= \abs{A^T y}$ in an optimal dual solution. Thus \eqref{dual LP} is equivalent to the right LP in \eqref{LP-Duality}.

\KM{Should we completely separate the two results?}

	We next show that the dual attains in minimum at a vertex of the feasible set. For this it suffices to show that its feasible set contains no line. Assume it does. Then there are vectors  $d = (y_1,\zp_1,\zn_1)$, $d$ non-zero, and $p = (y_0,\zp_0,\zn_0)$ such that $(y, \zp,\zn) = p + \lambda d = (y_0 + \lambda y_1, \zp_0 + \lambda \zp_1, \zn_0 + \lambda \zn_1)$ is feasible for all $\lambda \in \R$. Thus $\zp_1 = \zn_1 = 0$. Note that if either $\zp_1$ or $\zn_1$ would be non-zero then either  $\zp_0 + \lambda \zp_1$ or $\zn_0 + \lambda \zn_1$ would have a negative component for some lambda. Then $A^Ty + \zp + \zn = 0$ implies $A^Ty_1 = 0$. Since $A$ has full row rank, $y_1 = 0$. Thus the dual contains no line and the minimum is attained at a vertex of its feasible region. The feasible region of the dual does not depend on $x$. 

	Let $(y^1,\zp_1,\zn_1)$ to $(y^K,\zp_K,\zn_K)$ be the vertices of~\eqref{dual LP}, and let $D = \sset{\abs{A^T y^1},\ldots,\abs{A^T y^K}}$. For 
	\[
		x^\prime=\frac{x}{\min_{d \in D} d^T x}>0\quad\text{we have }\quad\min_{d \in D} d^T x^\prime = 1,
	\] and thus the right LP in \eqref{LP-Duality} has objective value 1. Hence, there is a feasible $f$ with $\abs{f} \le x^\prime$.
\end{proof}

Next, we give a similar result for the the directed case. Let $\alpha>0$, we define
an \emph{$\alpha$-weakly dominating set} by
$\mathcal{X}^{W}(\alpha):=
    \{ x\in\R^m:\exists\text{ feasible }f:0\le f \le \alpha x\}$.
\textcolor{red}{%
Note that for each $x>0$ there exists $\alpha>0$ such that $x$ belongs to the $\alpha$-weakly dominating set, and that the set of feasible points is a subset of $\mathcal{X}^W(1)$. Thus, as $\alpha$ increases, we obtain a gradually looser  relaxation of the notion of feasible point.  
}%(textcolor)

\begin{lemma}\label{lem_prDualLPs}
    For any $x \in \R_{>0}^{m}$ and $\alpha>0$, it holds that
	\begin{align}\label{directed LP-Duality}
        \min\{0:Af=b,0\leq f\leq\alpha x\}=\max\{b^{T}y
       -\alpha x^{T}\max\{0,A^{T}y\}:y\in\mathbb{R}^{n}\}.
   \end{align}
    Moreover, let $\mathcal{P}:=\{(y,z)\in\mathbb{R}^{n+m} :
    z\ge\max\{0,A^{T}y\},\|y\|_{\infty}\le1,\ b^{T}y\ge0\}$ be a polyhedron
    and $D'$ be the finite set of vertices of $\mathcal{P}$.
    Then, $x\in\mathcal{X}^{W}(\alpha)$ iff
    $b^{T}y\le\alpha x^{T}\max\{0,A^{T}y\}$ for every vertex $(y,z)\in D'$.
\end{lemma}
\begin{proof}
	The minimization problem can be written as
	\begin{align}
		\min\ \left\{ 0 : \begin{bmatrix}A & 0 \\
		I                              & I
		\end{bmatrix}\begin{bmatrix}f\\
		s
		\end{bmatrix}=\begin{bmatrix}b\\
		\alpha x
		\end{bmatrix}\text{ and }f,s\geq0\right\} .\label{LPMin}
	\end{align}
	Hence, its dual has unconstrained variables $y\in\R^n$ and $z\in\R^m$ and reads
	\begin{align}
		\max\left\{ \begin{bmatrix}b\\
		\alpha x
		\end{bmatrix}^{T}\begin{bmatrix}y\\
		z
		\end{bmatrix}:\begin{bmatrix}A^{T} & I \\
		0                                  & I
		\end{bmatrix}\begin{bmatrix}y\\
		z
        \end{bmatrix}\le 0\right\} =\max\left\{ b^{T}y-\alpha x^{T}z:z\ge\max\{0,A^{T}y\}\right\} .\label{LPMax}
	\end{align}
	The lower bound on $z$ is fulfilled with equality in any optimal
	solution since $x>0$. Thus the maximization problem can be written
	as $\max\{b^{T}y-\alpha x^{T}\max\{\mathbf{0},A^{T}y\}:y\in\mathbb{R}^{n}\}$,
	which establishes the first part of the lemma. For the second conclusion, notice that $x\in\mathcal{X}^{W}(\alpha)$ if and only
	if the optimum value of the primal-dual (\ref{LPMin},\ref{LPMax})
	equals 0, or equivalently
	\begin{align}
		\max\{b^{T}y-\alpha x^{T}z:z\ge\max\{\mathbf{0},A^{T}y\},\|y\|_{\infty}\le1,b^{T}y\ge0\}=0.\label{formula:maxproblem}
	\end{align}
	Since the polyhedron $\mathcal{P}$ does not contain a line and the
	optimum is finite, it follows that~\eqref{formula:maxproblem} has
	an extreme point that is optimal. \qedhere
\end{proof}

Inspired by this lemma, we define an \emph{$\alpha$-strongly dominating set} by
$\mathcal{X}(\alpha):=
    \{x\in\R_{\ge 0}:\alpha y^{T}Ax\ge b^{T}y\,\,\text{for every } (y,z)\in D'\}$.
By Lemma~\ref{lem_prDualLPs}, $\mathcal{X}(\alpha)\subseteq\mathcal{X}^{W}(\alpha)$ and $\mathcal{X}(\alpha)\subseteq\mathcal{X}(\beta)$ for any
$0<\alpha\le\beta$.
%\textcolor{red}{%
%Thus, $\alpha$-strongly dominating points are a relaxation of the notion of a feasible point, but a strengthening of $\alpha$-weakly dominating point. 
%}%(textcolor)


